SoftZoo: A Soft Robot Co-design Benchmark For Locomotion In Diverse Environments

While significant research progress has been made in robot learning for control, unique challenges arise when simultaneously co-optimizing morphology. Existing work has typically been tailored for particular environments or representations. In order to more fully understand inherent design and performance tradeoffs and accelerate the development of new breeds of soft robots, a comprehensive virtual platform with well-established tasks, environments, and evaluation metrics is needed. In this work, we introduce SoftZoo, a soft robot co-design platform for locomotion in diverse environments. SoftZoo supports an extensive, naturally-inspired material set, including the ability to simulate environments such as flat ground, desert, wetland, clay, ice, snow, shallow water, and ocean. Further, it provides a variety of tasks relevant for soft robotics, including fast locomotion, agile turning, and path following, as well as differentiable design representations for morphology and control. Combined, these elements form a feature-rich platform for analysis and development of soft robot co-design algorithms. We benchmark prevalent representations and co-design algorithms, and shed light on 1) the interplay between environment, morphology, and behavior; 2) the importance of design space representations; 3) the ambiguity in muscle formation and controller synthesis; and 4) the value of differentiable physics. We envision that SoftZoo will serve as a standard platform and template an approach toward the development of novel representations and algorithms for co-designing soft robots' behavioral and morphological intelligence.

==> sandbox/tmp.tex <==
% \begin{table}[t] 
%     \centering
%     \caption{Benchmark.}
%     % \begin{adjustbox}{width=0.3\columnwidth}
%     \begin{tabular}{c|ccccccc}
%         \toprule
%         % & \multicolumn{7}{c}{\textbf{Movement Speed}} \\
%         {\textbf{Movement Speed}} & Ground & Ice & Wetland & Clay & Desert & Snow & Aquatic \\
%         \midrule
%         Baby Seal & \\
%         Caterpillar & \\
%         Fish & \\
%         Panda & \\
%         \bottomrule
%     \end{tabular}
%     % \end{adjustbox}
%     \label{tab:benchmark}
% \end{table}

% \begin{table}
%     \begin{minipage}{0.3\linewidth}
%         \caption{Representation of design space.}
%         \label{tab:design_repr}
%         \centering
%         \begin{tabular}{lc}
%             \toprule
%             Representation   & Performance  \\
%             \midrule
%             Particle          &   \\
%             Voxel             &   \\ 
%             \makecell[l]{Implicit\\Function} &   \\
%             SDF Basis         &   \\
%             \makecell[l]{Wasserstein\\Barycenter}     &  \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}\hfill
%     \begin{minipage}{0.7\linewidth}
%         \centering
%         \includegraphics[width=0.7\linewidth]{example-image}
%         \captionof{figure}{Design space representation}
%     \end{minipage}
% \end{table}


% Contribution:
% \begin{itemize}
%     \item A benchmark of soft robot co-design for locomotion in diverse environments.
%     \item Demonstrate the importance of search space design from the perspective of 3D representation learning.
%     \item Study the role of differentiable physics.
%     \item Interplay between morphology, policy learning, and emergent motions.
% \end{itemize}


% \begin{table}
%     \begin{minipage}{0.3\linewidth}
%         \caption{Representation of design space.}
%         \label{tab:design_repr}
%         \centering
%         \begin{tabular}{lc}
%             \toprule
%             Representation   & Performance  \\
%             \midrule
%             Particle          & 0.027 \\
%             Voxel             & 0.023 \\
%             \midrule
%             Implicit Function & 0.113 \\
%             Diff-CPPN         & 0.091 \\
%             \midrule
%             SDF Basis         & 0.152 \\
%             Wass-Barycenter     & 0.158 \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}\hfill
%     \begin{minipage}{0.6\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth]{asset/tmp/shape_demo}
%         \captionof{figure}{Design space representation}
%     \end{minipage}
% \end{table}

% \begin{table}
%     \caption{Representation of design space.}
%     \label{tab:design_repr}
%     \centering
%     \begin{tabular}{l|cc}
%         \toprule
%         Representation  & Structural Prior & Performance  \\
%         \midrule
%         Particle          & None & 0.027 \\
%         Voxel             & None & 0.023 \\
%         \midrule
%         Implicit Function & Spatial Smoothness & 0.113 \\
%         Diff-CPPN         & Spatial Smoothness & 0.091 \\
%         \midrule
%         SDF Basis         & Design Basis & 0.152 \\
%         Wass-Barycenter     & Design Basis & 0.158 \\
%         \bottomrule
%     \end{tabular}    
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{asset/tmp/shape_demo}
%     \captionof{figure}{Design space representation}
% \end{figure}

% Inspired by nature.
% IMPORTANT Why virtual environment? driving force for research. (Rapid testbed)

% Many living creatures manifest different behaviors in response to characteristics or challenges of their environments. More interestingly, the strategies developed to survive their habitats are often tightly connected to their morphological structure. Such an intertwined relationship between environment, morphology, and behavior can serve as an inspiring perspective of developing artificial agents with an unified consideration of both body and brain. To this end, soft robotics community has demonstrated, beyond merely policy learning, the potential of leveraging body shape and material properties to achieve a wide variety of tasks. In this work, we introduce a soft robot co-design (learning / optimization in both robot body and policy) platform for locomotion in diverse environments with a differentiable physic engine. We demonstrate a fascinating interplay between environment, robot body, and motion when achieving various locomotion tasks. Furthermore, we identify and investigate several challenges in soft robot co-design from the view of design space representation, ambiguity between design and control, and the role of differentiable physics. We envision the proposed platform will encourage an distinctive way of approaching policy learning and the development of novel representations and learning algorithms for soft robot co-design.

% Story:
% \begin{itemize}
%     \item Nature has incubated a wide variety of creatures that exhibit different levels of intelligence and distinct behaviors in order to survive and thrive.
%     \item How embodied agents interact with the environment depends on not only the brain but also the body, i.e., certain emergent behavior may be unique to certain morphology.
%     \item Further highlight the inter-dependency on environment.
%     \item Overall, sell the story that highlights the interplay between environment, morphology, policy learning, and emergent behaviors.
%     \item In this work, we focus on soft robot co-design for locomotion in diverse environments. Explain why focusing on soft-bodied agents? And why locomotion?
% \end{itemize}

% Contribution:
% \begin{itemize}
%     \item We introduce a platform of soft robot co-design with a differentiable physics engine for locomotion in diverse scenarios, including ground, ice, wetland, clay, desert, snow, and aquatic environments.
%     \item We demonstrate the interplay between environment, morphology, and robot motion.
%     \item We identify and study the challenges in soft robot co-design from various perspectives, including design space representation, ambiguity between design and control, and the role of differentiable physics.
% \end{itemize}



% Benchmark of diverse locomotion:
% \begin{itemize}
%     \item Figures for all environments.
%         \begin{itemize}
%             \item Regular ground.
%             \item Icy.
%             \item Snow.
%             \item Desert (sand).
%             \item Wetland (mud).
%             \item Swamp (plasticine).
%             \item Rubber (jelly).
%             \item Aquatic.
%             \item Subterrain.
%         \end{itemize}
%     \item Introduce tasks and metrics.
%         \begin{itemize}
%             \item Task: Going along a fixed direction. Metric: Average speed along the direction.
%             \item Task: Moving in circles. Metric: Average angular velocity.
%             \item Task: Waypoint following. Metric: Average displacement error.
%             \item Task: Velocity tracking. Metric: Average speed along the varying direction.
%             \item General metric: efficiency.
%         \end{itemize}
%     \item Different animals with manually-annotated muscle and report performance of (i) different environments (ii) different policy learning methods.
%         \begin{itemize}
%             \item Policy architecture: linear combination with bias on periodic function bases with different frequencies and phases.
%             \item Animals: Caterpillar, Earthworm, Walrus/Seal, Panda, Marmot, Fish.
%             \item Policy learning methods: RL, differentiable physics.
%         \end{itemize}
% \end{itemize}

% Interplay between morphology, policy learning, and emergent motions:
% \begin{itemize}
%     \item Qualitative analysis on benchmarking on different animals.
%         \begin{itemize}
%             \item Track 3D motion (trajectory) of different muscle group.
%             \item Measure resistance on robot body in forward direction.
%         \end{itemize}
%     \item Identify different types of motions.
%         \begin{itemize}
%             \item Crawling.
%             \item Swimming.
%             \item Running.
%             \item Hopping.
%         \end{itemize}
%     \item Discuss connection between locomotion behaviors and environments.
% \end{itemize}

% Search space design based on 3D representation learning:
% \begin{itemize}
%     \item In aquatic environments, consider (i) passive dynamics (ii) fixed periodic controller and muscle.
%     \item Consider task of moving forward with metrics including forward speed and efficiency.
%     \item Use differentiable physics for optimization.
%     \item Compare shape search space with different structural priors:
%         \begin{itemize}
%             \item Particle-based representation.
%             \item Voxel-based representation.
%             \item MLP implicit function.
%             \item Diff-CPPN.
%             \item Wasserstein barycenter.
%             \item Base shape SDF interpolation.
%         \end{itemize}
%     \item Include task performance and learning efficiency.
% \end{itemize}

% Challenges in muscle placement and actuation:
% \begin{itemize}
%     \item Highlight the ambiguity between muscle placement and control in optimization.
%     \item Show muscle stiffness is a static version of actuation.
%     \item Show that with fixed shape, we can roughly approximate arbitrary muscle placement by redundant muscle setup with soft actuation mapping.
% \end{itemize}

% Study the role of differentiable physics:
% \begin{itemize}
%     \item Briefly discuss how differentiable physics is studied in the context of policy learning (no need of experiments since many other papers already did a lot of analysis).
%     \item Show loss landscape with respect to a single parameter (of morphology) in worst case,
%         \begin{itemize}
%             \item Shape: A box can fall to the right or to the left due to a single piece of corner being absent or not.
%             \item Softness: With the same contraction behavior, softer body can jump higher to pass a stump and show that there is a cusp between whether you can successfully pass the stump; this is a bit similar to discontinuity mentioned in the ICML diff-sim for control paper (from Russ's group) but here we highlight that controller depends on robot design and this is a similar observation yet from different angle.
%         \end{itemize}
% \end{itemize}

% Comparison of co-design methods:
% \begin{itemize}
%     \item Consider full co-design pipeline, including .
%     \item Focus on two environments: (i) regular land (ii) aquatic. 
%     \item Methods:
%         \begin{itemize}
%             \item CPPN-NEAT.
%             \item RL + NN policy and designer.
%             \item Function basis + differentiable physics.
%         \end{itemize}
%     \item This probably won't yield super meaningful results since it is probably too computationally intractable to actually do straightforward computational co-design in 3D simulation with complex environments and robot body. This is more of making the paper complete and we leave this to future exploration.
% \end{itemize}


\begin{table}[t] 
    \centering
    \caption{Large-scale benchmark of biologically-inspired designs in \namenospace. Each entry shows results from differentiable physics (left) and RL (right). The higher the better.}
    \vspace{-1mm}
    \begin{adjustbox}{width=1\columnwidth}
    \begin{tabular}{c|c|ccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Animal}} & \multicolumn{7}{c}{\textbf{Environment}} \\
        & & \textbf{Ground} & \textbf{Ice} & \textbf{Wetland} & \textbf{Clay} & \textbf{Desert} & \textbf{Snow} & \textbf{Ocean} \\
        \midrule 
        \multirow{4}{*}{\makecell{Movement\\Speed}} & Baby Seal & \textbf{0.122} / 0.241 & \textbf{0.048} / 0.013 & 0.032 / 0.026 & 0.012 / 0.007 & 0.059 / 0.019 & 0.039 / 0.011 & 0.033 / 0.003  \\
        & Caterpillar & 0.080 / 0.068 & 0.023 / 0.002 & \textbf{0.052} / 0.018 & 0.032 / 0.004 & 0.053 / 0.038 & 0.047 / 0.009 & 0.134 / \textbf{0.174} \\
        & Fish & 0.053 / 0.025 & 0.029 / 0.012 & 0.026 / 0.014 & \textbf{0.037} / 0.018 & \textbf{0.115} / 0.015 & \textbf{0.087} / 0.074 & 0.084 / 0.128 \\
        & Panda & 0.046 / 0.026 & 0.038 / 0.000 & 0.016 / 0.008 & 0.019 / 0.005 & 0.023 / 0.008 & 0.031 / 0.006 & 0.024 / 0.007 \\
        \midrule
        \multirow{4}{*}{Turning} & Baby Seal & 0.067 / \textbf{0.083} & \textbf{0.058} / 0.014 & 0.014 / 0.009 & 0.021 / 0.016 & \textbf{0.051} / 0.009 & 0.047 / 0.018 & 0.059 / 0.052 \\
        & Caterpillar & 0.053 / 0.016 & 0.021 / 0.011 & \textbf{0.040} / 0.007 & \textbf{0.027} / 0.005 & 0.034 / 0.005 & \textbf{0.069} / 0.015 & \textbf{0.195} / 0.115 \\
        & Fish & 0.032 / 0.064 & 0.023 / 0.005 & 0.023 / 0.009 & 0.015 / 0.004 & 0.021 / 0.013 & 0.028 / 0.014 & 0.041 / 0.020 \\
        & Panda & 0.064 / 0.037 & 0.023 / 0.004 & 0.009 / 0.004 & 0.008 / 0.001 & 0.014 / 0.003 & 0.013 / 0.003 & 0.035 / 0.034 \\
        \midrule
        \multirow{4}{*}{\makecell{Velocity\\Tracking}} & Baby Seal & 0.343 / 0.501 & 0.257 / 0.136 & 0.249 / 0.235 & 0.231 / 0.246 & 0.290 / 0.261 & 0.215 / 0.223 & 0.379 / 0.252 \\
        & Caterpillar & 0.502 / 0.312 & 0.101 / 0.343 & 0.426 / 0.240 & 0.282 / 0.072 & 0.441 / 0.308 & 0.379 / -0.113 & 0.555 / \textbf{0.739}  \\
        & Fish & 0.216 / 0.382 & 0.416 / 0.204 & 0.221 / 0.271 & 0.234 / \textbf{0.343} & \textbf{0.457} / 0.205 & \textbf{0.638} / 0.330 & 0.657 / 0.455 \\
        & Panda & \textbf{0.575} / 0.415 & \textbf{0.555} / 0.495 & \textbf{0.536} / 0.429 & 0.153 / 0.134 & 0.450 / -0.249 & 0.472 / 0.266 & 0.395 / 0.404 \\
        \midrule
        \multirow{4}{*}{\makecell{Waypoint\\Following}} & Baby Seal & -0.012 / -0.010 & -0.018 / -0.023 & -0.018 / -0.027 & \textbf{-0.020} / -0.026 & -0.012 / -0.027 & -0.014 / -0.025 & -0.010 / -0.026 \\
        & Caterpillar & -0.013 / -0.021 & -0.019 / -0.029 & \textbf{-0.016} / -0.028 & \textbf{-0.020} / -0.027 & -0.013 / -0.026 & -0.018 / -0.028 & \textbf{-0.002} / -0.023 \\
        & Fish & -0.004 / -0.029 & -0.016 / -0.024 & -0.022 / -0.033 & -0.024 / -0.031 & \textbf{-0.007} / -0.032 & \textbf{-0.003} / -0.023 & -0.005 / -0.023 \\
        & Panda & \textbf{-0.003} / -0.014 & \textbf{-0.014} / -0.023 & -0.021 / -0.026 & -0.023 / -0.028 & -0.010 / -0.021 & -0.008 / -0.026 & -0.013 / -0.025 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:benchmark}
    \vspace{-5mm}
\end{table}

==> source/scratch_chainqueen_math.tex <==
%\newcommand{\D}{\mathrm{d}}
\newcommand{\D}[1]{\frac{\partial L}{\partial {{#1}}}}
\newcommand{\pd}[2]{\frac{\partial{#1}}{\partial{#2}}}
%\newcommand{\chain}[2]{\D{#1}\cdot\pd{#1}{#2}}
\newcommand{\chain}[2]{\D{#1} \pd{#1}{#2}}
\newcommand{\dep}{\leftarrow}
\newcommand{\rdep}{\rightarrow}
\newcommand{\ttau}{\boldsymbol{\tau}}
\newcommand{\Dinv}{\frac{4}{\Delta x^2}}
\newcommand{\ePpn}{\PP_p^n & = & \PP_p^n(\FF_p^n, E_p, \nu_p)+\FF_p\sig_{pa}^n}
\newcommand{\emin}{m_i^{n} & = & \sum_p N(\xx_i-\xx_p^n)m_p}
\newcommand{\eppin}{\pp_i^{n} & = & \sum_p N(\xx_i- \xx_p^n) \left[m_p\vv_p^n+\left(-\Dinv\Delta t V_p^0\PP_p^n\FF_p^{nT} + m_p \CC_p^n\right)(\xx_i-\xx_p^n)\right]}
\newcommand{\evvin}{\vv_i^{n} & = & \frac{1}{m_i^n}\pp_i^n}
\newcommand{\evvpnn}{\vv_p^{n+1} & = & \sum_i N(\xx_i- \xx_p^n)\vv_i^n}
\newcommand{\eCCpnn}{\CC_p^{n+1} & = &\frac{4}{\Delta x^2} \sum_i N(\xx_i- \xx_p^n)\vv_i^n(\xx_i-\xx_p^n)^T}
\newcommand{\eFFpnn}{\FF_p^{n+1} & = & (\II + \Delta t \CC_p^{n+1})\FF_p^n}
\newcommand{\exxpnn}{\xx_p^{n+1} & = & \xx_p^n + \Delta t \vv_p^{n+1}}

\item \textbf{Particle-to-grid transfer (P2G).}
Particles transfer mass $m_p$, momentum $(m\vv)_p^n$, and stress-contributed impulse to their neighbouring grid nodes, using the Affine Particle-in-Cell method (APIC)~\cite{jiang2015} and moving least squares force discretization~\cite{hu2018moving}, weighted by a compact B-spline kernel $N$: ($\GG_p^n$ below is a temporary tensor)
\small
\begin{eqnarray}
%\ePpn \\
\emin,\\
\GG_p^n&=&-\Dinv\Delta t V_p^0\PP_p^n\FF_p^{nT} + m_p \CC_p^n,\\
\small\pp_i^{n} & = & \sum_p N(\xx_i- \xx_p^n) \left[m_p\vv_p^n+\GG_p^n(\xx_i-\xx_p^n)\right].
\end{eqnarray}
\normalsize
\vspace{-8pt}
\item \textbf{Grid operations.} Grid momentum is normalized into grid velocity after division by grid mass: \begin{eqnarray}\label{eqn:grid}
\evvin.
\end{eqnarray}
Note that neighbouring particles interact with each other through their shared grid nodes, and collisions are handled automatically. Here we omit boundary conditions and gravity for simplicity.
\item \textbf{Grid-to-particle transfer (G2P).} Particles gather updated velocity $\vv_p^{n+1}$, local velocity field gradients $\CC_p^{n+1}$ and position $\xx_p^{n+1}$. The constitutive model properties (e.g. deformation gradients $\FF_p^{n+1}$) are updated.

\small
\begin{eqnarray}
\evvpnn, \\
\eCCpnn, \\
\eFFpnn, \\
\exxpnn.
\end{eqnarray}
\normalsize

\end{enumerate}

\paragraph{Bonudary conditions (Contact models)} ChainQueen adopts four commonly used MPM boundary conditions from computer graphics~\cite{stomakhin2013material}. These boundary contidions happen on the grid, after Eqn. \ref{eqn:grid}. Denoting the grid node velocity as $\vv$ and local boundary normal as $\nn$, the four boundary conditions are
\begin{enumerate}
    \item[\textbf{Sticky}] Directly set the grid node velocity to $\mathbf{0}$. I.e., $\vv \leftarrow \mathbf{0}$.
    \item[\textbf{Slip}] Set the normal component of the grid node velocity to $0$. I.e., $\vv \leftarrow \vv - (\vv \cdot \nn)\nn$.
    \item[\textbf{Separate}] If the velocity is moving away from the boundary $(\vv \cdot \nn > 0)$ then do nothing. Otherwise use \textbf{Slip}. This can be considered as a special case (coefficient of friction $=0$) of \textbf{Friction}.
    \item[\textbf{Friction}] If the velocity is moving away from the boundary $(\vv \cdot \nn > 0)$ then do nothing. Otherwise apply Coulomb's law of friction to compute the new tangential and normal components of velocity after collision and friction.
\end{enumerate}

\subsection{Material Models}
We extend ChainQueen's original material model, which was simply fixed corotated material, in order to further support Neohookean materials as well.  We emphasize that other material models can be simply, modularly added as an option in ChainQueen, so long as they are differentiable.

\aes{The difference between Neohookean, corotated, and linear materials has been well studied and documented \cite{bonet1997nonlinear, liu2017quasi, smith2018stable}, especially in the static load case.  We direct the reader to the accompanying video, for a simple example of material model choice on a nearly incompressible oscillating actuator, demonstrating a modest, but not insignificant effect that choice of material model can have on a soft robot's dynamical response.  The (wall-time) difference in the computational cost of the Neohookean and corotated models is negligible.}

\paragraph{Fixed Corotated}  The fixed corotated material model~\cite{stomakhin2012energetically} is defined as having first Piola-Kirchoff Stress function $\PP$:

\begin{align}
\PP(\FF) = 2 \mu (\FF-\RR) + \lambda (J-1)J \FF^{-T}
\end{align}

\noindent where $J = \det(\FF)$, and $\lambda$ and $\mu$ are the first and second Lam\'e parameters, determined by the material's Young's modulus and Poisson's ratio.  Here, $\mathbf{R}$ is the rotational component of $\FF$, computable \emph{via} the (differentiable) polar decomposition.

\paragraph{Neohookean}  The Neohookean material \aes{model} is especially popular in modeling nonlinear rubbers and silicones.  The Neohookean elastic stress tensor is defined as:

\begin{align}
    \PP(\FF) = \mu(\FF - \FF^{-T}) + \lambda \log(J) \FF^{-T}
\end{align}

Although this energy model possesses a pole at $J=0$, this corresponds to the situation where the material is compressed to a singularity.  \aes{While instability caused by this singularity can happen in practice in general, it rarely occurs in the types of systems explored here, and never happened in any of our experiments.}  \footnote{Note that in MPM the update of $J$ (i.e. $\textbf{det}(F)$) is multiplicative instead of additive; getting $J \le 0$ \aes{is rare in our domain.  Inversions are still a serious topic of investigation for many other applications in MPM and MPM at large.}}

\paragraph{Incompressible materials}
\label{sec:incompressible}
Materials may be made approximately incompressible by adding a stress, as described by Bonet and Wood \cite{bonet1997nonlinear}.  In this scenario, an additional incompressibility stress tensor is added to the original stress tensor: $\PP = \PP_{elastic} + \PP_{inc}$:

\begin{align}
    \PP_{inc}(\FF) = \frac{E}{3 (2 - 2 \nu)} p (J - 1)^{p-1} J \FF^{-T}
\end{align}

\noindent where $p$ is a parameter $ \geq 2$.  The larger $p$ is chosen, the more strongly incompressibility will be enforced.  The ability to simulate incompressible materials is included in our ChainQueen extensions.

\subsection{Actuation Models}
\label{sec:actuation}
Designed to model real-world soft robots, our extended ChainQueen implementation supports two common actuation models found in soft robots.  The first, aimed at modeling fluidic actuators, is a stress-based actuation model.  The second, which we present here and aimed at modeling cable-based actuation, is a force-based actuation model.  These models are physically based and do not inject any net fictitious forces or pressures to the system (thus respecting Newton's third law).  We modify the classical MLS-MPM formulation with two additional steps in order to account for application of the actuation.

In order to model stress-based (including fluidic) actuators, we have designed an actuation model that stretches a given particle $p$ with an additional cauchy stress:
\begin{align}
\AA_p=\FF_p\sig_{pa}^{}\FF_p^T
\end{align}

Here, $\sig_{pa}=\text{diag}(a_x, a_y, a_z)$.  This equation corresponds to the stress in material space.  Particles corresponding to a given actuator are assigned at robot design time; each actuator thus affects many corresponding particles applying the same stress.  Note that this formulation naturally allows for both isotropic and anisotropic pressure actuators, useful for modeling directionally constrained actuators (\emph{e.g.} Sun et al \cite{sun2016miniature}).  Already, this model is well-suited for modeling stress-based actuators (\emph{e.g.} Hara et al \cite{hara2004artificial}) and pneumatic actuators (\emph{e.g.} Marchese et al\cite{marchese2015recipe}).  This model is similarly well-suited to simulating hydraulic actuators, modeling the actuator's particles as incompressible, as previously described in Section \ref{sec:incompressible}.

In order to model force-based actuators, such as cable-driven actuators, we simply integrate these forces when updating our particle velocity, creating an additional summable velocity term, $\mathbf{v}_{act}$:

\begin{align}
    \mathbf{v}_{act} = \mathbf{f}_{act} dt \aes{ / m}
\end{align}

\aes{Velocities, forces, and masses here refer to particle states.}  Here, $\mathbf{f}_{act}$ is computed as some user-defined force model.  We detail one such model here, which also provides a concrete example of how actuation signals can be applied. 

